Does Label Differential Privacy Prevent Label Inference Attacks?

Label differential privacy (label-DP) is a popular framework for training private ML models on datasets with public features and sensitive private labels. Despite its rigorous privacy guarantee, it has been observed that in practice label-DP does not preclude label inference attacks (LIAs): Models trained with label-DP can be evaluated on the public training features to recover, with high accuracy, the very private labels that it was designed to protect. In this work, we argue that this phenomenon is not paradoxical and that label-DP is designed to limit the advantage of an LIA adversary compared to predicting training labels using the Bayes classifier. At label-DP $\epsilon=0$ this advantage is zero, hence the optimal attack is to predict according to the Bayes classifier and is independent of the training labels. Our bound shows the semantic protection conferred by label-DP and gives guidelines on how to choose $\varepsilon$ to limit the threat of LIAs below a certain level. Finally, we empirically demonstrate that our result closely captures the behavior of simulated attacks on both synthetic and real world datasets.

==> sections/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}



==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
%connection with the pitfall paper

\citet{busa2021pitfalls} first realized the fact that even with the LDP guarantee, an adversary can still recover the training labels via the simple prediction attack. Their Bayesian interpretation of this paradox is that the public release of features contributed to this privacy loss and that LDP cannot mitigate this risk. We offer a different view and advocate that label leakage in absolute terms should not be considered a privacy violation. Instead, with the appropriate metric of success for the adversary, \emph{i.e.}, advantage, we showed that LDP can indeed prevent label inference attacks. We hope that future work can build upon our analysis to deepen our understanding of the connection between LDP and LIAs.

%a tighter bound
%a better dp-logloss tradeoff in Criteo dataset, previous algorithms focus too much on classification problems. benchmark.

==> sections/old_experiment.tex <==
\subsection{Experiments on Recommendation Datasets}
\label{sec:real_exp}
\paragraph{Datasets.} We experiment with recommendation dataset: LF-AmazonTitles-131K \cite{mcauley2013hidden}, LF-WikiSeeAlsoTitles-320K \cite{Bhatia16} and LF-AmazonTitles-1.3M \cite{mcauley2015image}. 
LF-AmazonTitles-131K and LF-AmazonTitles-1.3M are product-to-product datasets. LF-WikiSeeAlsoTitles-320K is a webpage-to-webpage dataset. The features are all bag of words. Those datasets additionally provide bag of words embeddings for labels from the same word dictionaries. The statistics of those datasets are listed in \autoref{tab:stats_data}.

\begin{table*}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|ccccc}
        \toprule
         & \# Train data & \# Distinct Training Features  & \# Test data & \# Distinct Test Features & $|\calY|$\\
        \midrule 
        LF-AmazonTitles-131K   & 674,996 & 294,805 & 284,746 & 134,835 & 131,073 \\
        LF-WikiSeeAlsoTitles-320K   & 1,460,012 & 693,082 & 540,833 & 177,515 & 312,330\\
        LF-AmazonTitles-1.3M & 49,911,367 & 2,248,619 & 16,138,900 & 970,237 & 1,305,265\\
        \bottomrule
    \end{tabular}
    }
    \caption{Statistics of the recommendation datasets. Some products / wikipedia-pages have more than one labels, so we also list the number of distinct features for both training set and test set. The attack advantage is evaluated per data and the model utility is average precision among distinct products / wikipedia-pages.}
    \label{tab:stats_data}
\end{table*}

\paragraph{Label DP algorithms.} We experiment with LP-MST and PATE-FM for all datasets. We choose DECAF, one of the state-of the-art extreme classification method, as the base non-private method.
Because those methods are mostly evaluated on image classification datasets not the extreme classification datasets, we make following adaptions for LP-MST and PATE-FM.
\begin{itemize}[leftmargin=*,nosep]
    \item LP-MST: Between stages, LP-MST needs a predicted probability vector among the label space by the learned model. Different from classification problem that probability vector is learned naturally from cross entropy loss, DECAF uses the most widely-used loss for extreme classification -- binary cross entropy loss, which generates semantic $\bbP(y=1|\bx)$ for each $y\in\calY$. To generate the probability, we further normalize the $(\bbP(y=1|\bx):y\in\calY)$ as the probability vector. 
    Moreover, LP-MST uses Mix-up \cite{zhang2018mixup} to train the classifier, which is robust to the label noise. However, the label noise in extreme classification is under-researched. Therefore we only follow the vanilla training from DECAF. We will discuss the literature of label noise in extreme classification in \autoref{sec:related_work}. 
    Furthermore, we also implement LP-MST with domain prior. This domain prior probability vector is computed as a normalized vector $\left(\langle \bx, \bv_y\rangle: y\in\calY\right)$, where $\bv_y$ is the bag of word feature for label $y$.
    
    \item PATE-FM: To make single prediction in the voting stage, we pick $\argmax_{y\in\calY}\bbP(y=1|\bx)$ as the single label prediction. The original paper PATE-FM uses the semi-supervised learning method for the training of both teachers and the student. As semi-supervised learning in extreme classification is under-researched, we only train DECAF with labeled data.
\end{itemize}

Overall, we experiment with LP-1ST, LP-2ST, LP-1ST ({\small domain prior}) and PATE-FM.

\paragraph{Attack algorithm.} We define $\calA^{\rm att}$ as $\calA(\calK)_i = \argmax_{y\calY} S_f(\bx_i, y)$, where $S_f(\bx_i, y)$ is the score that $f$ assigns to class $y$ given the feature $\bx$.

\paragraph{Evaluations.} We use prec@1 and prec@5 to evaluate the model utility. We define the benefit function $g(y^{\rm att}, y) :=\mathds{1}\{y^{\rm att} = y\}$ and the corresponding advantage function is ${\rm adv}(\calA^{\rm att}, \calK) = \frac{1}{n}\sum_{i=1}^n\bbE_{\by_i}\mathds{1}\{\calA^{\rm att}(\calK))_i = \by_i\}$.
As we don't have the label distribution as well, we evaluate the advantage for adversaries by $\frac{1}{n}\sum_{i=1}^n\mathds{1}\{\calA^{\rm att}(\calK))_i = \by_i\}$ instead.

\begin{table*}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|ccccccccc}
        \toprule
         Dataset & Method & & $\varepsilon=\infty$ & $\varepsilon=14$ & $\varepsilon=12$ & $\varepsilon=10$ & $\varepsilon=8$ & $\varepsilon=4$ & $\varepsilon=2$ & $\varepsilon=1$\\
        \midrule 
        \multirow{8}{*}{LF-AmazonTitles-131K}   & \multirow{2}{*}{LP-1ST} & Prec@1 / Prec@5 & 38.4 / 18.7 & 36.4 / 17.6 & 29.0 / 13.5 & 12.6 / 5.7 & 3.7 / 2.0 & 1.6 / 1.2 & 1.6 / 1.2 & 1.6 / 1.2  \\
        & & {Adv. of Attack} & 42.2 & 40.5 & 31.3 & 10.6 & 1.8 & 0.0 & 0.0 & 0.0 \\
        \cmidrule{2-11}
         & \multirow{2}{*}{LP-2ST} & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
         \cmidrule{2-11}
         & \multirow{2}{*}{LP-1ST ({\small domain prior})}  & Prec@1 / Prec@5 & - & 31.3 / 14.2 & 30.6 / 13.8 & 27.4 / 12.2 & 23.3 / 10.2 & 15.8 / 7.3 & 15.2 / 7.6 & 15.3 / 7.9 \\
         & & {Adv. of Attack} & - & 31.6 & 30.4 & 26.1 & 20.5 & 11.2 & 10.3 & 11.7 \\
         \cmidrule{2-11}
         & \multirow{2}{*}{PATE-FM}  & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
         
        \midrule 
        \multirow{8}{*}{LF-WikiSeeAlsoTitles-320K}   & \multirow{2}{*}{LP-1ST}& Prec@1 / Prec@5 &  & 22.5 / 11.2 & 14.5 / 6.9 & 7.2 / 3.8 & 4.3 / 2.6 & 3.5 / 2.2 & 3.4 / 2.1 & 3.4 / 2.2 \\
         & & {Adv. of Attack} & &40.3 & 23.7 & 8.6 & 4.9 & 4.1 & 4.0 & 3.9 \\
        \cmidrule{2-11}
         & \multirow{2}{*}{LP-2ST} & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
         \cmidrule{2-11}
         & \multirow{2}{*}{LP-1ST ({\small domain prior})}  & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
         \cmidrule{2-11}
         & \multirow{2}{*}{PATE-FM}  & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
        \midrule 
        \multirow{8}{*}{LF-AmazonTitles-1.3M}   & \multirow{2}{*}{LP-1ST} & Prec@1 / Prec@5 &  & & & & & & &  \\
         & & {Adv. of Attack} & & & & & & & &  \\
        \cmidrule{2-11}
         & \multirow{2}{*}{LP-2ST} & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
         \cmidrule{2-11}
         & \multirow{2}{*}{LP-1ST ({\small domain prior})}  & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
         \cmidrule{2-11}
         & \multirow{2}{*}{PATE-FM}  & Prec@1 / Prec@5 & - & & & & & & &  \\
         & & {Adv. of Attack} & - & & & & & & &  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Model utility and attack advantage with different $\varepsilon$. We report Prec@1 / Prec@5 for model utility and the inferance accuracy for the attack advantage.}
    \label{tab:real_world_results}
\end{table*}

\paragraph{Results.} \autoref{tab:real_world_results} shows the results.

==> sections/problem_setting_old.tex <==
% \section{Problem Set-up}
\section{Does Label-DP Prevent Label Inference Attacks?}
\label{sec:setup}

\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
    \toprule
       \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{2}{c}{\textbf{MNIST} ($\varepsilon=1.0$)} & \multicolumn{2}{c|}{\textbf{MNIST} ($\varepsilon=0.1$)} & \multicolumn{2}{c}{\textbf{CIFAR10} ($\varepsilon=1.0$)} & \multicolumn{2}{c}{\textbf{CIFAR10} ($\varepsilon=0.1$)} \\
    \cmidrule{2-9}
        & Test Acc. & Attack Acc. & Test Acc. & Attack Acc. & Test Acc. & Attack Acc. & Test Acc. & Attack Acc. \\
    \midrule
       LP-1ST & 93.3 & 93.3 & 20.8 & 20.9 & 61.5 & 61.9 & 15.5 & 15.8\\
       LP-1ST ({\small in-domain prior})  & 97.1 & 96.5 & 97.0 & 96.2 & 75.4 & 75.7 & 66.3 & 66.3 \\
       LP-1ST ({\small out-of-domain pior}) & 94.6 & 93.7 & 86.2 & 85.2  & 89.5 & 89.8 & 87.6 & 86.9 \\
       PATE-FM & 99.3 & 99.1 & 23.6 & 23.0 & 92.4 & 92.1 & 18.6 & 18.6 \\
       ALIBI & 96.3 & 96.3 & 21.5 & 20.8 & 67.5 & 69.6 & 13.6 & 13.9 \\
    %   ClusterRR & & & & & & & & \\
    \bottomrule
    \end{tabular}
    }
    \caption{Model test accuracy and attack accuracy of the simple prediction attack (SPA) evaluated on label-DP models trained on MNIST and CIFAR10. SPA attack accuracy is equivalent to training accuracy for classification and is exceptionally high in most cases. Our evaluation shows that a learning algorithm can offer a very stringent label-DP guarantee of $\varepsilon=0.1$ while failing to prevent label inference attacks.}
    \label{tab:empi_eval_ldp_algo}
    \vspace{-2ex}
\end{table*}

Relaxing DP to label-DP provided the flexibility for designing more specialized private learning algorithms. These methods seem to provide excellent trade-offs between privacy and model utility, as measured by their high test accuracy even at very low $\varepsilon$, $\delta$ values.
In this section, we take a closer look at the privacy protection offered by label-DP. We argue that not only is label-DP unable to prevent adversaries from inferring the training labels under arbitrarily low values of privacy parameter $\varepsilon > 0$, \emph{any} model that generalizes will inevitably fail to do so as well.

\subsection{Existing Label Inference Attack against Label-DP}
\label{sec:paradox_label_dp}

% Practical Label DP algorithms exist
%Several recent publications~\cite{ghazi2021deep, esmaeili2021antipodes, esfandiari2021label} have introduced practical machine learning algorithms that adhere to the label DP framework (Definition~\autoref{def:label_dp}).

% But they do not protect you from an adversary finding out the label


\paragraph{Label Inference Attack in Vertical Federated Learning.} In the setting of \textit{Vertical Federated Learning} (VFL), one party has the features and the other party has the labels. Two parties want to train a model together without leaking the privacy of data. The party with features holds the first several layers of the model and the party with labels have the remaining layers of the model. \cite{sun2022label} shows that even when the label-DP ($\varepsilon=0.5$) is applied in the VFL, under their proposed label inference attack, the party with the features and the first several model layers can achieve AUC 0.75 of label leakage.


\paragraph{Label Inference Attack in Label-DP Model Training.} We first make the observation that the label-DP guarantee \emph{does not} imply that an adversary cannot leverage the model to infer its training labels. In fact, if the training accuracy is high, the adversary can trivially evaluate the model on the public training set and recover its labels~\cite{busa2021pitfalls}. We refer to this attack as the \emph{simple prediction attack} (SPA) and evaluate it on existing label-DP learning algorithms.

%The results confirm this speculation: even though these models achieve great utility on benchmark image datasets, the simple prediction attack from these models achieves very high attack accuracy too.

% Several recent work study label DP algorithms for model release, which are LP-MST \cite{ghazi2021deep}, PATE-FM \cite{esmaeili2021antipodes} and ALIBI \cite{esmaeili2021antipodes}. 
% For LP-MST, we especially evaluate LP-1ST with no prior, prior estimated from same public training features and prior estimated from extra out-domain features trained from ImageNet \cite{deng2009imagenet}. % and ClusterRR \cite{esfandiari2021label}.
% They show decent accuracy at small DP parameter $\varepsilon$ on MNIST \cite{lecun1998gradient} and CIFAR10  \cite{krizhevsky2009learning}. 
% We can check the those columns of accuracy in \autoref{tab:empi_eval_ldp_algo}. 
% When $\varepsilon=1.0$ or $0.1$, the accuracy could be as high as $97.1$ and $97.0$ in the experiment of MNIST, and $92.4$ and $87.6$ in the experiment of CIFAR10.%which borrows the out-domain knowledge: it utilizes the feature extractor trained from ImageNet \cite{deng2009imagenet}.
% \todo{update the results.} 

% We conduct some experiments to show this
%We refer to this attack as the \emph{simple prediction attack} and evaluate it on current state-of-the-art label DP algorithms: LP-MST, PATE-FM, and ALIBI.


% For LP-MST,  % and ClusterRR \cite{esfandiari2021label}.
% we especially evaluate LP-1ST with no prior, prior estimated from same public training features and prior estimated from extra out-domain features trained from ImageNet \cite{deng2009imagenet}.
% They show decent accuracy at small DP parameter $\varepsilon$ on MNIST \cite{lecun1998gradient} and CIFAR10  \cite{krizhevsky2009learning}. 
% We can check the those columns of accuracy in \autoref{tab:empi_eval_ldp_algo}. 
% When $\varepsilon=1.0$ or $0.1$, the accuracy could be as high as $97.1$ and $97.0$ in the experiment of MNIST, and $92.4$ and $87.6$ in the experiment of CIFAR10.

% Because the setting of label privacy assumes features are publicly available data, a simple attack is to predict the labels from the features by the released model. 
% We name this attack as \emph{simple prediction attack}. 
% We measure the accuracy of such an attack as the amount of label privacy leakage. 
% We evaluate the label privacy leakages for 4 label DP algorithms. 
% Results in \autoref{tab:empi_eval_ldp_algo} show that under the strong guarantee of label DP  $(\varepsilon=0.1)$, the label privacy leakage is surprisingly severe: the accuracy of the attack is such high as $96.2$ (MNIST) and $86.9$ (CIFAR10).
% \todo{update the numbers later}

\autoref{tab:empi_eval_ldp_algo} shows test accuracy for several label-DP models trained on MNIST~\cite{lecun1998gradient} and CIFAR10~\cite{krizhevsky2009learning}, along with the corresponding SPA attack accuracy, \emph{i.e.}, the model's training accuracy. There is a clear trend that these algorithms can achieve very high test accuracies with strong label-DP guarantee, \emph{i.e.}, low privacy parameter $\varepsilon$.
%with strong DP guarantee i.e. small DP parameter $\varepsilon$, these algorithms achieve high test accuracy on MNIST \cite{lecun1998gradient} and CIFAR10 \cite{krizhevsky2009learning} in \autoref{tab:empi_eval_ldp_algo}.
%These algorithms show decent accuracy at small DP parameter $\varepsilon$ on MNIST \cite{lecun1998gradient} and CIFAR10 \cite{krizhevsky2009learning} in \autoref{tab:empi_eval_ldp_algo}. 
For instance, at $\varepsilon=0.1$, the test accuracy could reach as high as $97.0$ for MNIST and $87.6$ for CIFAR10.
However, the SPA attack accuracy is almost identical to the model's test accuracy, which (paradoxically) seems to suggest that models leak a tremendous amount of label information even when trained with stringent label-DP guarantees.
%We also measure the accuracy of a simple prediction attack, i.e. the accuracy on the training set, as the amount of label privacy leakage.
%Results in \autoref{tab:empi_eval_ldp_algo} show that under the strong guarantee of label DP  $(\varepsilon=0.1)$, the label privacy leakage is still surprisingly severe: the accuracy of the attack is as high as $96.2$ (MNIST) and $86.9$ (CIFAR10).
%Moreover, notice that the gap between model accuracy and leakage is very small. We will discuss this point in detail in the next subsection.

\subsection{Impossibility of Label Protection under Label-DP}
\label{sec:impossibility_ldp}

Following the above observation, a natural question to ask is whether the vulnerability of label-DP to the existing label inference attack is due to an insufficiently strong privacy guarantee, \emph{i.e.}, $\varepsilon,\delta$ being not small enough. We give a definitive negative answer by formalizing \emph{label inference attacks} (LIAs) and showing that label-DP cannot guarantee protection against LIAs even for arbitrarily small values of $\varepsilon,\delta > 0$.

\paragraph{Threat model.}
The adversary's goal is to design a label inference attack algorithm $\calA$ that infers the training label of each sample in the training dataset.
%We define the label inference attack $\calA^{\rm att}$, with which the adversaries attempt to infer the label for each training data point from their best knowledge. Formally the output of any label inference attack
The output of $\calA$ is a vector of inferred labels $\hat{\by} \in \calY^{n}$. We assume that the adversary has access to the following information:
%We define what knowledge the adversary has as below:
\begin{enumerate}[leftmargin=*,nosep]
    \item The adversary has full knowledge of the model $f = \calM(X, \by)$, where $\calM$ is the training algorithm, since $f$ is released publicly in the setting of label privacy.
    \item The adversary has full knowledge of the public feature matrix $X\in\bbR^{n\times d}$.
    \item (Optional) The adversary has knowledge of the conditional data distribution $\bbP(y|\bx)$ of $\calD$.
    %It is similar to the setting of membership inference attack \cite{yeom2018privacy}. 
\end{enumerate}
We refer to the threat model with or without the third assumption as the \emph{with-prior} or \emph{priorless} setting. The with-prior setting is not unrealistic: Given access to a separate dataset for the same learning task, the adversary can train a shadow model to estimate the conditional probability $\bbP(y|\bx)$. Such an approach is commonly used in membership inference attacks~\cite{shokri2017membership}.
%when the adversary has a model trained on a different dataset but for the same task, this model might have good transferability to the to-be-trained dataset and strongly indicates $\bbP(y|\bx)$ for the dataset that we want to protect.

\paragraph{Expected attack utility.} To measure how successful an LIA is at inferring training labels, we define the \emph{attack utility function} $u(\hat{\by}_i, \by_i)$ where $\hat{\by}_i \in \calY$ is the inferred label and $\by_i$ is the ground truth. We assume that $u(\hat{\by}_i, \by_i) \in [0,B]$ for any $\hat{\by}_i, \by_i \in \calY$,
%The adversary wants to infer the training data's labels $\by$. Denote label inference algorithm as $\calA^{\rm att}$, which outputs the inferred labels $\by^{\rm att} \in \calY^n$. We define the attack utility function as $g(\by^{\rm att}_i, \by_i)$ and assume its value is bounded between $0$ and $B$ for any $\by^{\rm att}_i, \by_i\in \calY$.
\emph{e.g.}, $u(\hat{\by}_i, \by_i)=\mathds{1}(\hat{\by}_i = \by_i)$ is the zero-one accuracy for classification problems, which is bounded with $B=1$. For regression problems with bounded label range $\calY\subseteq [-b, b]$, we can define $u(\hat{\by}_i, \by_i) = 4b^2 - (\hat{\by}_i - \by_i)^2$, which is bounded with $B=4b^2$. We assume $B=1$ for simplicity; our results can be easily generalized to any $B > 0$.

The \emph{expected attack utility} (EAU) is defined as the expectation of $u(\hat{\by}_i, \by_i)$ over the randomness of the sampling of labels and in the learning algorithm:
\begin{equation}
\label{equ:adv}
    \mathrm{EAU}(\calA, \calK) = \bbE_{\by,\calM}\left[ \left. \frac{1}{n} \sum_{i=1}^n u(\hat{\by}_i, \by_i ) \right| X\right],
\end{equation}
where $\calK$ denotes the adversary's knowledge: $(X, f, \bbP(y|\bx))$ for the with-prior setting and $(X, f)$ for the priorless setting.

\paragraph{Upper bound on expected attack utility.}
For attack utility functions $u$ that reflect the accuracy of a label inference attack, one may ask whether label-DP can provide a uniform upper bound $U(\varepsilon, \delta)$ such that
\begin{equation}
\label{equ:uniform_bound}
    \mathrm{EAU}\left(\calA, \calK\right) \leq U(\varepsilon, \delta)
\end{equation}
holds for any data distribution $\calD$, feature matrix $X$ and attack algorithm $\calA$.
A trivial upper bound $U(\varepsilon, \delta) \leq 1$ follows from the boundedness of $u$.
Unfortunately, we show that this bound is in fact optimal for both the with-prior and the priorless settings.

\begin{theorem}
\label{thm:upper_bound}
There is no function $U(\varepsilon,\delta)$ that satisfies \autoref{equ:uniform_bound} and is strictly less than $1$ at some $\varepsilon, \delta>0$.
\end{theorem}
\begin{proof}
We first consider the with-prior setting where the adversary has access to the conditional distribution $\bbP(y|\bx))$. For a classification problem with utility function $u(\hat{\by}_i, \by_i)=\mathds{1}(\hat{\by}_i = \by_i)$, we define the attack $\calA_{\rm prior}$ that predicts training labels according to the Bayes classifier:
\begin{equation}
\label{equ:prior_att}
\calA_{\rm prior}(\calK) := \left(\argmax_{y\in\calY}\bbP(\by_i=y|X_i): i=1, \cdots n\right).
\end{equation}
The expected attack utility for $\calA_{\rm prior}$ is:
\begin{equation}
\label{equ:prior_adv}
    \mathrm{EAU}\left(\calA_{\rm prior}, \calK\right) = \frac{1}{n}\sum_{i=1}^n\max_{y\in\calY}\bbP(\by_i=y|X_i).
\end{equation}
In particular, when the label $y$ is deterministic given the feature $\bx$, \emph{i.e.}, $\bbP(y|\bx) = 1$ for some $y \in \calY$, this EAU evaluates to $1$. Note that $\calA_{\rm prior}$ does not depend on $f$ and is thus valid for any $\varepsilon, \delta$, hence $U(\varepsilon, \delta)\geq 1 ~\forall \varepsilon, \delta>0$.

For the \emph{priorless} setting, consider again a classification problem with the same utility function $u$. Denote by $\calA_{\rm priorless}$ the simple prediction attack, which predicts labels using the trained model $f$.
We will construct a series of settings ($\calD^n$, $X^n$, $f^n$) such that each $f^n$ is $(\varepsilon, \delta)$-label-DP and as $n\to \infty$, ${\rm \text{EAU}}\left(\calA_{\rm priorless}, \calK\right) \to 1$, which shows that $U(\varepsilon, \delta)\geq 1 ~\forall \varepsilon, \delta>0$.
\begin{itemize}[leftmargin=*,nosep]
    \item \emph{Data construction}: The feature domain $\calX$ is $\{-1, 1\}$ and the label space $\calY$ is $\{-1, 1\}$. We construct $X^n$ with $n = 2r$ samples where $X_1^n= \cdots = X_r^n = 1$ and $X_{r+1}^n = \cdots = X_{2r}^n = -1$. The conditional label distribution given the feature is $\bbP(\by_i^n = X_i^n | X_i^n) = 1$ for all $i$.
    \item \emph{Label-DP algorithm for training $f^n$}: We apply randomized response with $\bbP(\tilde{\by}_i = \by_i^n) = \frac{e^{\varepsilon}}{e^{\varepsilon} + 1}$ to privatize the labels. We then train $f^n$ on the privatized labels to maximize training accuracy, which results in $f^n$ being simply the majority sign function: $f^n(1) = \text{sign}\{ \sum_{i=1}^r \tilde{\by}_i \}$ and $f^n(-1) = \text{sign}\left\{ \sum_{i=r+1}^{2r} \tilde{\by}_i \right\}$.
\end{itemize}
The fact that $f^n$ is $(\varepsilon, 0)$-label-DP follows from $\tilde{\by}_i$ being the randomized response of $\by_i$ for $i=1,\ldots,n$ and $f^n$ being a post-processing function. The SPA attack's EAU is equal to the training accuracy of the model $f^n$, which can be lower bounded using Hoeffding's inequality:
\begin{align*}
    &\hspace{3ex} \bbE\left[ \left. \frac{1}{n} \sum_{i=1}^n \calA_{\rm priorless}(X^n, f^n)_i = \by_i^n \right| X^n \right] \\
    &= \frac{1}{2} \cdot \bbP\left( \sum_{i=1}^r \tilde{\by}_i >0\right) + \frac{1}{2} \cdot \bbP\left( \sum_{i=r+1}^{2r} \tilde{\by}_i <0\right)\\
    &\geq  \bbP\left( \left|\frac{1}{r}\sum_{i=1}^r \frac{1 + \tilde{\by}_i}{2} - \frac{e^{\varepsilon}}{e^{\varepsilon} + 1}\right| \leq \frac{e^{\varepsilon}}{e^{\varepsilon} + 1}  - \frac{1}{2}  \right) \\
    &\geq 1 - 2\exp\left(-\left(\frac{e^{\varepsilon}}{e^{\varepsilon} + 1} - \frac{1}{2}\right)^2 n\right).
\end{align*}
Taking $n \rightarrow \infty$ gives the desired result.
%Then we are able to show $U(\varepsilon, \delta)\geq 1$ for any $\varepsilon>0$:
%\begin{align*}
%&U(\varepsilon, \delta)\geq \lim_{n\to \infty}{\rm \text{EAU}}\left(\calA^{\rm att}_{\rm priorless}, \calK^n\right)\\
%&\lim_{r\to \infty}\frac{1}{n}\sum_{i=1}^{n}\bbP(\calA^{\rm att}_{\rm priorless}(X^n, f)_i = \by_i^n | X^n) = 1.
%\end{align*}
\end{proof}

\autoref{thm:upper_bound} shows that for both the with-prior and priorless settings, no non-trivial upper bound for EAU exists for any label-DP privacy parameters $\varepsilon,\delta>0$. It also validates our rationalization about the experimental result in \autoref{tab:empi_eval_ldp_algo} that failure to prevent the SPA attack is to be expected.

%We showed that at both prior and priorless setting, $U(\varepsilon, \delta)$ that satisfies \autoref{equ:adv_upper} is no less than $1$. Thus the trvial upper bound $1$ is optimal for ${\rm \text{EAU}}\left(\calA^{\rm att}, \calK\right)$.
%It supports the experiment results in \autoref{tab:empi_eval_ldp_algo} because LDP has no meaningful guarantee for the expected attack utility, the failure of protect against the simple prediction attack is to be expected.
% This result also suggests that LDP may protect something different from the expected attack utility.

\subsection{Impossibility of Label Protection when Model Generalizes}
\label{sec:paradox_tradeoff}
% We discuss the possibility of utility-privacy trade-off for classification or regression tasks. 
% A natural question for the trade-off is raised: is it possible to have a model $f$ s.t. $f$ has \emph{test utility} higher than $a_1$ but the \emph{label privacy leakage} is limited by $a_2$? 
% Formally the \emph{test utility} is defined as $a_1:=\bbE_{(\bx, y)\sim \calD} u(f(\bx), y)$ where $u:\calY\times \calY\to \bbR_{\geq 0}$ is any utility function. 
% For example, when we define $u(y^{\rm pred}, y)$ as $\mathds{1}\{y^{\rm pred}= y\}$, the test  utility $\bbE_{(\bx, y)\sim \calD} u(f(\bx), y)$ is test accuracy.
% The \emph{label privacy leakage} in this section refers to the utility of \emph{simple prediction attack}, which could be formally written as $a_2:=\frac{1}{n}\sum_{i=1}^n u(f(X_i), \by_i)$.
% Notice that the label privacy leakage is equivalent to the training accuracy of the model. 

% Given $\Delta > 0$, we will discuss several common conditions, under which it would be very unlikely that $f$ has utility as high as $a_1$ but has relatively smaller label privacy leakage $a_2\leq a_1-\Delta$, where the randomness comes from the training set sampling process and the training process.
% These conditions are highly related to the generalization bound.
% We put the derivations of the conclusions below into the appendix.

% The first type of conditions follows the classical uniform convergence results. We summarize the conclusions for both binary classification and multi-class classification as below:
% \begin{itemize}[leftmargin=*,nosep]
%     \item \textbf{Binary classification:} Suppose the binary classifier $f$ is learned from a hypothesis space $\calH$ with \emph{finite} VC dimension $\VCD$ \cite{vapnik1999nature}. Then,
%     $$
%     \bbP(a_1 - a_2 \geq \Delta)\leq \exp\left(\VCD - Cn\Delta^2\right)
%     $$
%     for some universal constant $C>0$.
    
%     \item \textbf{Multi-class classification:} Suppose the multi-class classifier $f$ is learned from a hypothesis space $\calH$ with \emph{finite} Natarajan dimension $d_N$ \cite{natarajan1989learning, bendavid1995characterizations}. 
%     Then,
%     $$
%     \bbP(a_1 - a_2 \geq \Delta)\leq \exp\left(d_N\log|\calY| - Cn\Delta^2\right)
%     $$
%     for some universal constant $C>0$.
    
%     \item \textbf{Regression:} Consider a real-value function $f$ is learned from a hypothesis space $\calH$ with \emph{finite} pseudo-dimension $\text{Pdim}$ \cite{anthony1999learning}. 
%     Assume $u(y^{\rm pred}, y)$ is bounded in $[-b, b]$ and is $L$-Lipschitz in $y^{\rm pred}$.
%     Then,
%     \begin{align*}
%         \bbP(a_1 - a_2 \geq \Delta) \leq 4\left(\frac{8L}{\Delta}\right)^{\text{Pdim}}\exp\left(-n\Delta^2/128b^2\right)
%     \end{align*}
% \end{itemize}
% For all cases, we draw the conclusion that when the hypothesis is ``simple" and training set size $n$ is large enough, it is unlikely that $a_1 - a_2 > \Delta$.

% The second condition comes from the generalization property implied by differential privacy. Assume $u(y^{\rm pred}, y)$ is bounded in $[0, 1]$. If $f$ is trained differentially privately with $(\varepsilon, \delta)$, $\bbE[a_1 - a_2] \leq 1-(1-\delta)e^{-\varepsilon}$. We can then draw the conclusion that when $(\varepsilon, \delta)$ is strong enough, it is impossible that the $\bbE[a_1 - a_2] > \Delta$. Notice that DP algorithms are all label DP algorithms. This fact implies that stronger guarantee of (label) DP (smaller $\varepsilon$ and $\delta$) sometimes makes larger scope of trade-offs impossible.

% We discuss the utility-privacy trade-off for machine learning tasks, including both classification and regression. When the privacy leakage and model utility have the same metrics, e.g. the accuracy in the discussion in the last subsection, the trade-off is highly related to the model generalization --  the gap between the performance on the training set and the test set. When generalization gap is guaranteed to be small, it sounds unachievable that in the end the model has high performance on test set, but limited leakage on the training set -- it not only holds potentially for models with label DP, but holds for any model with the generalization property. We summarize some generalization results next.W

While the statement of \autoref{thm:upper_bound} may suggest that label-DP is an insufficient notion of label privacy, we argue that a similar conclusion can be made about \emph{any} reasonable learning algorithm. In particular, the ubiquitous desirable property that the model \emph{generalizes} is in fact in conflict with the goal of limiting the expected attack utility of an LIA.

For both classification and regression problems, a natural choice for the attack utility function is the model utility---zero-one accuracy for classification and (negative) squared error for regression. In this case, EAU for the SPA attack is exactly the model's utility on the training set. If the model generalizes then the train-test utility gap must be small, hence it is impossible to simultaneously attain a high test accuracy for the model and a low EAU for the SPA attack. We highlight two particularly contradictory scenarios for which generalization leads to vulnerability to LIAs.

%We discuss whether it is achievable of any privacy-utility trade-off for machine learning tasks in the setting of label-only privacy, where the privacy here indicates the attack utility of \emph{simple prediction attack}. When the attack utility and model utility have the same metrics, e.g. the accuracy in the discussion in the last subsection, the trade-off is identical to the model generalization --  the gap between the performance on the training set and the test set. When generalization gap is guaranteed to be small, it sounds unachievable that in the end the model has high performance on test set, but limited leakage on the training set -- it not only holds potentially for models with label DP, but holds for any model with the generalization property. We summarize some generalization results next.

% The generalization could be guaranteed by the probability uniform convergence bound given from statistical learning. Classical results show the generalization bound for binary classification \cite{vapnik1999nature}, multi-class classification \cite{natarajan1989learning, bendavid1995characterizations} and regression \cite{anthony1999learning} problems. From these results, it's guaranteed that with high probability the generalization gap for \emph{any} model is small, when the hypothesis complexity (VC dimension, Natarajan dimension or pseudo dimension) is limited and the size of training set is large enough.

\paragraph{Generalization for low-capacity models.} Classical learning theory asserts that if the hypothesis class for the learning algorithm has limited capacity, \emph{e.g.}, low VC dimension~\cite{vapnik1999nature} or Natarajan dimension~\cite{natarajan1989learning} for binary/multi-class classification and low pseudo-dimensionality~\cite{anthony1999learning} for regression, then generalization follows by uniform convergence for \emph{any} learning algorithm. Such a result is counter-intuitive to the common belief that privacy leakage is primarily due to memorization in high-capacity models~\cite{feldman2020does}.
%When models are with low capacity, they are vulnerable to the simple prediction attack \emph{no matter how models are trained}. Classic results show the strong generalization bound for binary classification \cite{vapnik1999nature}, multi-class classification \cite{natarajan1989learning, bendavid1995characterizations} and regression \cite{anthony1999learning} problems.

\paragraph{Generalization via differential privacy.} It can be shown that differential privacy can also reduce the train-test utility gap, leading to higher EAU for the SPA attack.
Dwork et al.~\cite{dwork2015preserving} showed that when the utility function $u$ is bounded between $[0, 1]$, the train-test utility gap is upper bounded by $e^{\varepsilon} - 1 + \delta$. We improve this upper bound to $1- \frac{2}{1 + e^{\varepsilon}} (1-\delta)$ in the theorem below; proof is given in \autoref{app:derivations}.
\begin{theorem}
\label{thm:dp_generalization}
Let $\calA$ be an $(\varepsilon, \delta)$-differentially private learning algorithm, and let $f = \calA(X, \by)$ be a model trained on the dataset $(X, \by)$. Let $u(y', y):\calY \times \calY \to [0, 1]$ be the utility function. Let $(\bx, y)$ be an independent random sample from the data distribution $\calD$. Then,
\resizebox{\linewidth}{!}{
  \begin{minipage}{\linewidth}
\begin{align*}
\left|\frac{1}{n}\sum_{i=1}^n\bbE[u(f(X_i), \by_i)] - \bbE[u(f(\bx), y)]\right| \leq 1-  \frac{2}{1 + e^{\varepsilon}} (1 - \delta).
\end{align*}
\end{minipage}
}
\end{theorem}
% When models are trained differentially privately, it seems DP contrarily guarantees the success of the simple prediction attack --- \citet{wang2016learning, wu2019generalization} show that differential privacy guarantees the model generalization too.

\autoref{thm:dp_generalization} yields a particularly contradictory conclusion: The privacy protection offered by DP results in better model generalization, but in turn makes it impossible to prevent training label leakage for high-utility models.
In fact, such a result is in-line with the design principle of DP as not to prevent statistical inference~\cite{mcsherry2016statistical, bun2021statistical}; that is, a model that generalizes merely performs statistical inference on the training data and does not leak any private information. Consequently, we argue that \emph{one should not equate label privacy with reducing the attacker's utility in absolute terms}.

% Differential privacy implies the generalization too\todo{add citation}. Explicitly, if a model is guaranteed to be $(\varepsilon, \delta)$-differentially private, the performance between train and test is bounded by $1 - (1-\delta)e^{-\varepsilon}$ for any utility function between $[0, 1]$. 

% \subsection{Problem Set-Up}
% Firstly, with strong label DP guarantee, a simple prediction attack possibly has high accuracy successfully predicts the labels correctly in the experiments of CIFAR10 and MNIST. Secondly, under some conditions of hypothesis space and enough training samples, with very few probability, any model, including the model trained with label DP, can achieve such a trade-off that the test utility is $a_1$ but the simple prediction attack for training labels has utility $a_2\leq a_1 - \Delta$. Thirdly, algorithm with strong enough differentially private guarantee makes the trade-off $\bbE[a_2]\leq \bbE[a_1] - \Delta$ impossible.

% These discussions raise two questions naturally: 
% \begin{enumerate}
%     \item \emph{Does label differential privacy protect label privacy?}
%     \item \emph{Is there a scenario where the model utility is satisfied and the privacy leakage is limited? Could label differential privacy help with it?}
% \end{enumerate}
% We will answer question 1 in \autoref{sec:label_dp} and question 2 in \autoref{sec:tradeoff_discussion}.

%\subsection{Summary}
%We summarize two paradoxes. Firstly, with strong label DP guarantee, the attacker is able to successfully predicts the labels mostly correct, which is justified in the experiments of CIFAR10 and MNIST. Secondly, it seems impossible to have great model utility and privacy protection together as long as the model has generalization property, while on the other hand the generalization is persued by machine learning community all the time. 

% These discussions raise one questions naturally: \emph{does label differential privacy prevent label inference attack?}
%These discussions raise one question naturally: \emph{does label differential privacy prevent label inference attack?} We answer this question in the next section.
% We will answer question 1 in \autoref{sec:label_dp} and question 2 in \autoref{sec:tradeoff_discussion}.

==> sections/tradeoff_discussion.tex <==
% \section{Existence of the Trade-off between Label Privacy and Model Utility}
\section{Trade-off between Label Privacy and Model Utility in the Real World}
\label{sec:tradeoff_discussion}
% \paragraph{Could label DP help achieve any satisfying trade-off?} 
Recall that in section \ref{sec:paradox_tradeoff} we discuss the trade-off between the model's \emph{test utility} $\bbE_{(\bx, y)\sim \calD}u(f(\bx), y)$ for some utility function $u$, and the expected attack utility $\bbE\left[\frac{1}{n}\sum_{i=1}^n g(\calA^{\rm att}(X, f)_i, \by_i)\right]$, with $\calA^{\rm att}(X, f)_i = f(X_i)$ and $g=u$. %With the generalization guarantee, 
In the other word, with a high test utility model, the labels wouldn't be protected \emph{if the attack utility function $g$ is equal to the utility function $u$}, which is also justified by the experiments for CIFAR10 and MNIST in \autoref{sec:setup}.
%when the attack utility function $g$ equals to the utility function $u$ and the $\calA^{\rm att}$ is \emph{simple prediction attack}.
Nevertheless, in the real world application, we have larger scope of satisfying model utility when the simple prediction attack has small expected attack utility, 
%the utility of model is satisfying in practice and at the meantime the labels could be protected, which we say this trade-off is \emph{satisfactory in practice}:
\begin{itemize}[leftmargin=*,nosep]
\item Some tasks do not require the model to have an absolute high utility value. In some cases, as long as the test utility could be higher than the random, such model could bring benefit to the company in practice, e.g. to predict if a stock is grown or predict which next product the user would be interested in. 
\item The attack utility function $g$ could be different from the utility function $u$. Because of the difference between $g$ and $u$, there is freedom that the utility among the test distribution is high but the advantage gained by adversaries is limited. For example, in a classification task, one reasonable utility function $u$ is to measures top-5 accuracy, while the advantage is defined as the (top-1) accuracy. It allows a classification model to have 0 top-1 accuracy but $100\%$ top-5 accuracy.
\end{itemize}
On the other hand, the result in \autoref{sec:label_dp} concludes that the label DP could guarantee the expected attack utility of any attack relative to the base advantage $\frac{1}{n}\sum_{i=1}^n\max_{y\in \calY}\bbE_{\by_i} \left[g(y, \by_i)|X_i\right]$. 

If for a task 1. the model utility does have larger scope of satisfying model utility and 2. the base advantage is a decent protection for label privacy, we can conclude that the trade-off between strict label DP guarantee and satisfying model utility is able to translate to a satisfying trade-off between label privacy evaluated by any label inference attack and the model utility. We next present a real world application which is exactly located in the setting of label privacy and meets 1 and 2 here.

\paragraph{A real world application for label DP.} 
% With the discussion above, because the base advantage is very high in the example of MNIST and CIFAR10, label DP cannot guarantee a great trade-off between label privacy and the test utility in this case.
% For the study of label privacy, we propose the product-to-product or webpage-to-webpage recommendation tasks as an appropriate scenario and suggest related datasets as the benchmark\todo{add citation}.
% In these tasks, we need to learn a model to recommend one or more potential products that the user is potentially interested in,  when an arbitrary user browsed or bought a specific product. 
For the study of label privacy, we propose the click-through rate (CTR) prediction, a part of Ads recommendation, as an appropriate application and suggest the related dataset as the benchmark.
In the CTR prediction, we need to learn a model to predict the probability that an impression with feature $\bx$, always a combination of product feature and user feature, will lead to click.

% Firstly, only labels are sensitive in such recommendation tasks.
% Denote $p$ as the product.
% The dataset consists of $n$ product pairs $(\bx, y)$, where $\bx$ is the feature of a product $p$ and $y$ is the index of the product $p'$ that a user next browsed / purchased after browsing / purchasing $p$.
% It's possible that $\bx$ is repeated but has different labels in different data.
% The feature $\bx$ in this dataset is publicly available.
% However the labels are usually sensitive -- they are collected by users' browsing / buying history.
% Firstly, only labels are sensitive. The product information and user information are accessible online, while the label $y$, whether click $(y=1)$ or not $(y=0)$, is sensitive -- it comes from the user click history.

% Secondly, a satisfying trade-off exists for those tasks. 
% The recommendation model, as discussed, is able to bring extra benefit to the company / user as long as it could beat the random recommendations. 
% Moreover, $g\neq u$ is the case. The utility function $u$ is usually set as precision \cite{gunawardana2009survey} \todo{add citation} for a learned \emph{scoring function}, while in the meaning of adversaries, the attack utility function $g$ measures the accuracy to infer the training labels.
In the CTR prediction task, we have larger scope of satisfying model utility. Firstly, the CTR model is able to bring extra benefit to the company / user as long as it could beat the random model.
Moreover, $g\neq u$ is the case. 
Log loss is usually used to evaluate the learned rate prediction model.
We take the negative of log loss as the utility function.
In the meaning of adversaries, however, the attack utility function $g$ measures the weighted accuracy to infer the training labels. 
The weight here captures that the data of label $y=1$ is more valuable than $y=0$ in the meaning of user privacy, because "what user is interested in" is more sensitive than "what user is not interested in".
Mathematically, $g(y^{\rm att}, y):=\frac{1}{2p_y}\mathds{1}\{y^{\rm att} = y\}$, where $p_1:=\bbP_{(\bx, y)\sim \calD}(y=1)$ is the probability that $y=1$ in the distribution $\calD$ and $p_0:=1-p_1$.

Moreover, the base advantage is likely not very large in this task.
As the attack utility function defined above, we can check the weighted accuracy of those naive solutions -- all 1 prediction, all 0 prediction or half-half random guess -- are all around $0.5$.
We hypothesis that the base advantage defined in the \autoref{equ:excess_adv} wouldn't be far away from $0.5$ and check this hypothesis in the experiment section. %which is relatively low compared to $1$ if the attacker predict each training label correctly and it should be a satisfying value in the sense of ``privacy".

% We hypothesis that the probability of the next browsed / purchased product will not concentrate on exact one product, but will be distributed on multiple products. With this hypothesis, the base advantage should be controlled below a satisfying value in the sense of ``privacy".

% We will experiment with several product / webpage recommendation datasets in \autoref{sec:real_exp}.
% The experiment results will show that although existed methods achieve nearly perfect trade-off between label DP and model accuracy in the experiments of MNIST and CIFAR10, their performances on those recommendation datasets suggests future efforts to improve the trade-off between the label DP parameters and the model utility.
% \todo{update the description of the experiment results}

We will experiment with a CTR prediction dataset provided by Criteo\footnote{\href{https://ailab.criteo.com/download-criteo-1tb-click-logs-dataset/}{https://ailab.criteo.com/download-criteo-1tb-click-logs-dataset/}} in \autoref{sec:real_exp}.
The experiment results will show that although existed methods achieve nearly perfect trade-off between label DP and model accuracy in the experiments of MNIST and CIFAR10, their performances on this CTR dataset suggests future efforts to improve the trade-off between the label DP parameters and the model utility.
